Comparative layer-wise analysis of self-supervised speech models

Many self-supervised speech models, varying in their pre-training objective, input modality, and pre-training data, have been proposed in the last few years. Despite impressive successes on downstream tasks, we still have a limited understanding of the properties encoded by the models and the differences across models. In this work, we examine the intermediate representations for a variety of recent models. Specifically, we measure acoustic, phonetic, and word-level properties encoded in individual layers, using a lightweight analysis tool based on canonical correlation analysis (CCA). We find that these properties evolve across layers differently depending on the model, and the variations relate to the choice of pre-training objective. We further investigate the utility of our analyses for downstream tasks by comparing the property trends with performance on speech recognition and spoken language understanding tasks. We discover that CCA trends provide reliable guidance to choose layers of interest for downstream tasks and that single-layer performance often matches or improves upon using all layers, suggesting implications for more efficient use of pre-trained models.

==> sections/outline.tex <==
\section{Outline}

In this work:
\begin{enumerate}
    \item layer-wise trends of properties contained in different pre-trained models: acoustic, phonetic, word identity, semantics; using a variety of tools
    \begin{enumerate}
        \item Effect of training data size, model size, pre-training objective
        \item Impact of visual grounding on these trends, in what aspects is the latter better/worse?
    \end{enumerate}
    \item (maybe) Address "did not consider de-localization effects" shortcoming in the previous work:
    \begin{enumerate}
        \item If majority of attention weight is *indeed* localized to diagonal elements: analysing just the localized extraction should be faithful to the actual content.
        \item We can consider adding just the preliminary analysis of attention weight matrices
    \end{enumerate}
    \item Layer importance for downstream tasks
    \ap{does this flow make sense?}
    \begin{enumerate}
        \item Assumption: "CCA-task and NC-task are indicative of layer-wise task specificity"
        \item Can we establish that downstream layer weights are indeed higher for more task-specific layers?
        \item Fine-tuning experiments for some task-model pair or for all tasks on a certain model
    \end{enumerate}
\end{enumerate}

\section{Results/Experiments}
\subsection{List of all models}
\ap{I think we should perform xlsr (and avhubert too?) experiments on dataset other than librispeech}
\begin{enumerate}
    \item Monolingual, effect of trainig objective
    \begin{enumerate}
    \item w2v2: base, large, vox
    \item hubert: base, large
    \item wavlm: base, base+, large
    \end{enumerate}
    \item Multilingual
    \begin{enumerate}
    \item xlsr: xlsr-53
    \end{enumerate}
    \item Multimodal
    \begin{enumerate}
    \item avhubert: base, large
    \item fastvgs: base, base+
    \end{enumerate}
\end{enumerate}
\subsection{Representation extraction}
\ap{New addition}
\begin{enumerate}
    \item Discuss normalization of extracted representations
    \item Preliminary findings from the analysis of attention weights
    \item In-depth analysis (including effect of fine-tuning and implications for fine-tuning) left for future work
\end{enumerate}
\subsection{Layer-wise property trends: analysis experiments}
\begin{enumerate}
    \item Model dynamics: cca\_intra
    \item Acoustics: cca\_mel
    \item Phonetics: cca\_phone\ap{the fact that hubert (and wavlm too?) show a saturating trend in the last few layers motivates us to analyze the clustered discrete units and if they provide any reasonable speech unit boundaries.}
    \item word: cca\_agwe, cca\_word, word discriminability\ap{vanilla experiments (not dtw and rnn variants)}
    \item Semantics: cca\_glove, WordSim\ap{need to convince ourselves first, choose a subset of tasks}, SpokenSTS\ap{yet to see the results}
\end{enumerate}
\subsection{Downstream tasks}
\begin{enumerate}
    \item Experiments w/ labeled classification data. \href{https://docs.google.com/spreadsheets/d/1lL3OE0h-dri1vSnsaizuDY2Y5jXluyNLBdRsqDzorqg/edit#gid=1287096029}{Link to the list of tasks}.
    \begin{enumerate}
        \item CCA w/ task labels, neural collapse \ap{can skip neural collapse?}
        \begin{itemize}
            \item Correlation of above with trends in sec 2.3
            \item Are different properties indicative of layer importance for different downstream tasks?
        \end{itemize}
        \item correlation of above with fine-tuning weights w/ frozen representations
        \item A light-weight fine-tuning strategy (similar to Hongyuan's work): for a specific task-model pair OR can leave as a suggestion, citing Hongyuan's work saying that similar ideas have worked for text models and tasks.\ap{But their paper may not be publicly available by the time we submit}
        \item In-depth experimentation (including generalizability of these strategies to different tasks and pre-trained pre-trained models) left for future work
    \end{enumerate}
\end{enumerate}
